Weak mu-equality is decidable

In this paper we consider the set of mu-types, an extension of the set of simple types freely generated from a set of atomic types and the type constructor ->, by a new operator mu, to explicitly denote solutions of recursive equations like A = A -> beta. We show that this so-called weak mu-equality for mu-types is decidable by defining a derivation system for weak mu-equality based on standard reduction for mu-types such that the number of nodes in a derivation tree for A = B is bounded as a function of A, B. We give two proofs. One for decidability of = for alpha-equivalence classes of mu-types and one for = for mu-types theselves. Both proofs are straightforward and elementary.

==> marcdef.tex <==
%LOGIC
\newcommand{\all}[2]{\forall#1\;#2}
\newcommand{\ex}[2]{\exists#1\;#2}
\newcommand{\allin}[3]{\forall#1\,{\in}\,#2\;#3}
\newcommand{\exin}[3]{\exists#1\,{\in}\,#2\;#3}
\newcommand{\allinm}[3]{\forall#1\,{\inm}\,#2\;#3}
\newcommand{\exinm}[3]{\exists#1\,{\inm}\,#2\;#3}
\newcommand{\longiff}{\mathrel{\;\;\iff\;\;}}
%\newcommand{\implies}{\Rightarrow}
\newcommand{\fT}{{\rightarrow}}
\newcommand{\ftO}{{\m_{\typO}}}
\newcommand{\fts}{{\m_A}}
\newcommand{\ftt}{{\m_B}}
\newcommand{\ftst}{{\m_{A\fT B}}}
\newcommand{\ftOO}{{\m_{\typO\fT\typO}}}
\newcommand{\longimplies}{\mathrel{\;\implies\;}}
\newcommand{\longneg}{\neg\;}
\newcommand{\Ter}{\mathit{Ter}}
%\newcommand{\Var}{\mathit{Var}}
\renewcommand{\Sub}{\mathit{Sub}}
\newcommand{\Ctx}{\mathit{Ctx}}
\newcommand{\Typ}{\mathit{Typ}}
%ORDINALS
\newcommand{\epsO}{\epsilon_0}
\newcommand{\oM}{\omega}
\newcommand{\empli}{[\,]}
%\renewcommand{\ord}[1]{{\underline{#1}}}
\renewcommand{\ord}[1]{{{#1}}}
\newcommand{\Qt}[1]{\overline{#1}}
%\newcommand{\Bar}[1]{\overline{#1}}
\newcommand{\OL}[1]{\overline{#1}}
\newcommand{\Fin}{\textrm{Fin}}
\newcommand{\Lim}{\textrm{Lim}}
\newcommand{\Succ}{\textrm{Succ}}
\newcommand{\Ord}{\textrm{Ord}}
\newcommand{\ordadd}{\textrm{plus}}
\newcommand{\ordmult}{\textrm{times}}
\newcommand{\ordexp}{\textrm{exp}}
\newcommand{\exptwo}{\textrm{exp2}}
\newcommand{\sord}{\textrm{succ}}
\newcommand{\pred}{\textrm{pred}}
\newcommand{\ap}{\textrm{p}}
\newcommand{\nm}{\textrm{num}}
\newcommand{\mun}{\textrm{mun}}
\newcommand{\pH}{\mathit{propH}}
%ARS NOTIONS
\newcommand{\UN}{{\rm UN}}
%\newcommand{\SN}{{\rm SN}}
%\newcommand{\WN}{{\rm WN}}
\newcommand{\tHF}{{\rm HF}}
\newcommand{\tHFc}{{\rm HF}^{0}}
\newcommand{\HF}{\mathscr{H\!F}}
%\newcommand{\HFc}{\mathscr{H\!F}^{0}}
\newcommand{\nf}{{\mathit{nf}}}
\newcommand{\Ind}{{\rm Ind}}
%\newcommand{\WCR}{{\rm WCR}}
%\newcommand{\CR}{{\rm CR}}
\newcommand{\WF}{{\rm WF}}
%\newcommand{\AC}{{\rm AC}}
\newcommand{\AF}{{\rm AF}}
%XY-DIAGRAM-ARROWS
\newcommand{\Onestep}{\ar@{>}}
\newcommand{\Manyred}{\ar@{>>}}
\newcommand{\Emptystep}{\ar@{.}}
\newcommand{\Symstep}{\ar@{|-|}}
\newcommand{\Line}{\ar@{-}}
\newcommand{\Noline}{\ar@{}}
\newcommand{\Dashed}{\ar@{--}}
\newcommand{\Manydots}{\ar@{.>>}}
\newcommand{\Onedots}{\ar@{.>}}
\newcommand{\Linedots}{\ar@{.}}
\newcommand{\Curldash}{\ar@{~~}}
\newcommand{\Linecurl}{\ar@{~}}
\newcommand{\Doubline}{\ar@{=}}
\newcommand{\lfrac}[2]{#1 \div #2}
\newcommand{\sfrac}[2]{\mbox{$\frac{#1}{#2}$}}
%MISCELLANEOUS
\newcommand{\sxy}{\textrm{sum}}
\newcommand{\cofs}{\,^{\underline{\,.\,}}\,}
%\newcommand{\lth}{\textrm{length}}
\newcommand{\If}{\textrm{If}}
\newcommand{\Ext}{\textrm{Ext}}
\newcommand{\lfp}{\textrm{lfp}}
\newcommand{\TIn}{\textrm{TI}}
\newcommand{\TIa}{\textrm{TI}_\a}
\newcommand{\TIc}{\textrm{TI}_\gamma}
\newcommand{\TIoM}{\textrm{TI}_\oM}
\newcommand{\TR}{\textrm{TR}}
\newcommand{\TRa}{\textrm{TR}_\alpha}
\newcommand{\TRoM}{\textrm{TR}_\oM}
\newcommand{\typO}{{\sf{N}}}
\newcommand{\baseT}{\om}
\newcommand{\oneT}{1}
\newcommand{\oneTone}{{\oneT\fT\oneT}}
\newcommand{\combI}{\comb{I}}
\newcommand{\combO}{\comb{0}}
\newcommand{\cL}{\comb{L}}
\newcommand{\cR}{\comb{R}}
\newcommand{\cI}{\comb{I}}
\newcommand{\combS}{{\comb{S}^{\!{+}}}}
\newcommand{\combR}{\comb{R}}
\newcommand{\combB}{\comb{B}}
\newcommand{\combY}{\comb{Y}}
\newcommand{\combE}{\comb{E}}
\newcommand{\Bc}{\comb{B}^{\!c}}
\newcommand{\nT}[1]{\comb{#1}}
\newcommand{\rT}{\red_{T}}
\newcommand{\rB}{\red_{B}}
\newcommand{\rY}{\red_{Y}}
\newcommand{\rE}{\red_{E}}
\newcommand\SP{\mathit{SP}}
\newcommand{\eSP}{=_{\be\mathit{SP}}}
\newcommand{\rSP}{\red_{\be\mathit{SP}}}
\newcommand{\rrSP}{\redd_{\be\mathit{SP}}}
\newcommand{\rbe}{\red_{\beta\eta}}
\renewcommand{\LT}{\Lambda_{T}}
\newcommand{\LTc}{\Lambda_{T}^{0}}
\newcommand{\LB}{\Lambda_{B}}
\newcommand{\LBc}{\Lambda_{B}^{0}}
\newcommand{\LY}{\Lambda_{Y}}
\newcommand{\LYc}{\Lambda_{Y}^{0}}
\newcommand{\LE}{\Lambda_{E}}
\newcommand{\LEc}{\Lambda_{E}^{0}}
\newcommand{\LSP}{\Lambda_{\mathit{SP}}}
\newcommand{\LSPc}{\Lambda_{\mathit{SP}^{0}}}
\renewcommand{\B}{\mathcal{B}}
\renewcommand{\Y}{\mathcal{Y}}
\renewcommand{\E}{\mathcal{E}}
%\newcommand{\calA}{\mathcal{A}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calF}{\mathcal{F}}
%\newcommand{\calX}{\mathcal{X}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\CmC}{{\cal C}}%{\mathcal{C\!\!\mathcal{C}}}
%\ltau,\lT,\lB,\lY in bk1.sty
\newcommand{\lE}{\l{E}}
\newcommand{\lSP}{\l_{\mathit{SP}}}
\newcommand{\HRO}{\mathit{HRO}}
\newcommand{\HEO}{\mathit{HEO}}
\newcommand{\CPO}{\mathit{CPO}}
\newcommand{\natbot}{\nat^{\bot}}
\newcommand{\HAw}{\hbox{\sf HA}^{\omega}}
\newcommand{\inseg}[2]{\overline{#1\,#2}} 

%\newcommand{\text}[1]{\mbox{\emph{#1}}}
\newcommand{\ssec}{\subsection*}
\newcommand{\sssec}{\subsubsection*}
\newtheorem{claim}{Claim}


%CALLIGRAPHIC
\newcommand{\mc}[1]{{\mathcal{#1}}}
\newcommand{\setA}{{\mathscr A}}
\newcommand{\setB}{{\mathscr B}}
\newcommand{\setBc}{{\mathscr B}^{\!c}}
\newcommand{\setC}{{\mathscr C}}
\newcommand{\setD}{{\mathscr D}}
\newcommand{\setG}{{\mathscr G}}
\newcommand{\setH}{{\mathscr H}}
\newcommand{\setM}{{\mathscr M}}
\newcommand{\setN}{{\mathscr N}}
\newcommand{\setT}{{\mathscr T}}
\newcommand{\setU}{{\mathscr U}}
\newcommand{\setV}{{\mathscr V}}
\newcommand{\setW}{{\mathscr W}}
\newcommand{\setX}{{\mathscr X}}
\newcommand{\setY}{{\mathscr Y}}
\newcommand{\setZ}{{\mathscr Z}}
\newcommand{\vecQ}{{\vec{Q}}}
\newcommand{\vecW}{{\vec{W}}}
\newcommand{\vecZ}{{\vec{Z}}}
\newcommand{\vecsetU}{{\vec{\mathscr U}}}
\newcommand{\vecsetW}{{\vec{\mathscr W}}}
\newcommand{\vecsetY}{{\vec{\mathscr Y}}}
\newcommand{\vecsetZ}{{\vec{\mathscr Z}}}



==> prooftree.tex <==
\message{<Paul Taylor's Proof Trees, 17 August 1990>}
%% Build proof tree for Natural Deduction, Sequent Calculus, etc.
%% WITH SHORTENING OF PROOF RULES!
%% Paul Taylor, begun 10 Oct 1989
%% *** THIS IS ONLY A PRELIMINARY VERSION AND THINGS MAY CHANGE! ***
%%
%%	\prooftree
%%		hyp1		produces:
%%		hyp2
%%		hyp3		        hyp1	hyp2	hyp3
%%	\justifies		        -------------------- rulename
%%		concl			           concl
%%	\thickness=0.08em
%%	\shiftright 2em
%%	\using
%%		rulename
%%	\endprooftree
%%
%% where the hypotheses may be similar structures or just formulae.
%%
%% To get a vertical string of dots instead of the proof rule, do
%%
%%	\prooftree			which produces:
%%		[hyp]
%%	\using					[hyp]
%%		name				  .
%%	\proofdotseparation=1.2ex		  .name
%%	\proofdotnumber=4			  .
%%	\leadsto				  .
%%		concl				concl
%%	\endprooftree
%%q

%% Within a prooftree, \[ and \] may be used instead of \prooftree and
%% \endprooftree; this is not permitted at the outer level because it
%% conflicts with LaTeX. Also,
%%	\Justifies
%% produces a double line. In LaTeX you can use \begin{prooftree} and
%% \end{prootree} at the outer level (however this will not work for the inner
%% levels, but in any case why would you want to be so verbose?).
%%
%% All of of the keywords except \prooftree and \endprooftree are optional
%% and may appear in any order. They may also be combined in \newcommand's
%% eg "\def\Cut{\using\sf cut\thickness.08em\justifies}" with the abbreviation
%% "\prooftree hyp1 hyp2 \Cut \concl \endprooftree". This is recommended and
%% some standard abbreviations will be found at the end of this file.
%%
%% \thickness specifies the breadth of the rule in any units, although
%% font-relative units such as "ex" or "em" are preferable.
%% It may optionally be followed by "=".
%% \proofrulebreadth=.08em or \setlength\proofrulebreadth{.08em} may also be
%% used either in place of \thickness or globally; the default is 0.04em.
%% \proofdotseparation and \proofdotnumber control the size of the
%% string of dots
%%
%% If proof trees and formulae are mixed, some explicit spacing is needed,
%% but don't put anything to the left of the left-most (or the right of
%% the right-most) hypothesis, or put it in braces, because this will cause
%% the indentation to be lost.
%%
%% By default the conclusion is centered wrt the left-most and right-most
%% immediate hypotheses (not their proofs); \shiftright or \shiftleft moves
%% it relative to this position. (Not sure about this specification or how
%% it should affect spreading of proof tree.)
%%==========================================================================

\def\introrule{{\cal I}}\def\elimrule{{\cal E}}%%
\def\andintro{\using{\land}\introrule\justifies}%%
\def\impelim{\using{\Rightarrow}\elimrule\justifies}%%
\def\allintro{\using{\forall}\introrule\justifies}%%
\def\allelim{\using{\forall}\elimrule\justifies}%%
\def\falseelim{\using{\bot}\elimrule\justifies}%%
\def\existsintro{\using{\exists}\introrule\justifies}%%

%% #1 is meant to be 1 or 2 for the first or second formula
\def\andelim#1{\using{\land}#1\elimrule\justifies}%%
\def\orintro#1{\using{\lor}#1\introrule\justifies}%%

%% #1 is meant to be a label corresponding to the discharged hypothesis/es
\def\impintro#1{\using{\Rightarrow}\introrule_{#1}\justifies}%%
\def\orelim#1{\using{\lor}\elimrule_{#1}\justifies}%%
\def\existselim#1{\using{\exists}\elimrule_{#1}\justifies}

%%==========================================================================

\newdimen\proofrulebreadth \proofrulebreadth=.05em
\newdimen\proofdotseparation \proofdotseparation=1.25ex
\newdimen\proofrulebaseline \proofrulebaseline=2ex
\newcount\proofdotnumber \proofdotnumber=3
\let\then\relax
\def\hfi{\hskip0pt plus.0001fil}
\mathchardef\squigto="3A3B
%
% flag where we are
\newif\ifinsideprooftree\insideprooftreefalse
\newif\ifonleftofproofrule\onleftofproofrulefalse
\newif\ifproofdots\proofdotsfalse
\newif\ifdoubleproof\doubleprooffalse
\let\wereinproofbit\relax
%
% dimensions and boxes of bits
\newdimen\shortenproofleft
\newdimen\shortenproofright
\newdimen\proofbelowshift
\newbox\proofabove
\newbox\proofbelow
\newbox\proofrulename
%
% miscellaneous commands for setting values
\def\shiftproofbelow{\let\next\relax\afterassignment\setshiftproofbelow\dimen0 }
\def\shiftproofbelowneg{\def\next{\multiply\dimen0 by-1 }%
\afterassignment\setshiftproofbelow\dimen0 }
\def\setshiftproofbelow{\next\proofbelowshift=\dimen0 }
\def\setproofrulebreadth{\proofrulebreadth}

%=============================================================================
\def\prooftree{% NESTED ZERO (\ifonleftofproofrule)
%
% first find out whether we're at the left-hand end of a proof rule
\ifnum	\lastpenalty=1
\then	\unpenalty
\else	\onleftofproofrulefalse
\fi
%
% some space on left (except if we're on left, and no infinity for outermost)
\ifonleftofproofrule
\else	\ifinsideprooftree
	\then	\hskip.5em plus1fil
	\fi
\fi
%
% begin our proof tree environment
\bgroup% NESTED ONE (\proofbelow, \proofrulename, \proofabove,
%		\shortenproofleft, \shortenproofright, \proofrulebreadth)
\setbox\proofbelow=\hbox{}\setbox\proofrulename=\hbox{}%
\let\justifies\proofover\let\leadsto\proofoverdots\let\Justifies\proofoverdbl
\let\using\proofusing\let\[\prooftree
\ifinsideprooftree\let\]\endprooftree\fi
\proofdotsfalse\doubleprooffalse
\let\thickness\setproofrulebreadth
\let\shiftright\shiftproofbelow \let\shift\shiftproofbelow
\let\shiftleft\shiftproofbelowneg
\let\ifwasinsideprooftree\ifinsideprooftree
\insideprooftreetrue
%
% now begin to set the top of the rule (definitions local to it)
\setbox\proofabove=\hbox\bgroup$\displaystyle % NESTED TWO
\let\wereinproofbit\prooftree
%
% these local variables will be copied out:
\shortenproofleft=0pt \shortenproofright=0pt \proofbelowshift=0pt
%
% flags to enable inner proof tree to detect if on left:
\onleftofproofruletrue\penalty1
}

%=============================================================================
% end whatever box and copy crucial values out of it
\def\eproofbit{% NESTED TWO
%
% various hacks applicable to hypothesis list 
\ifx	\wereinproofbit\prooftree
\then	\ifcase	\lastpenalty
	\then	\shortenproofright=0pt	% 0: some other object, no indentation
	\or	\unpenalty\hfil		% 1: empty hypotheses, just glue
	\or	\unpenalty\unskip	% 2: just had a tree, remove glue
	\else	\shortenproofright=0pt	% eh?
	\fi
\fi
%
% pass out crucial values from scope
\global\dimen0=\shortenproofleft
\global\dimen1=\shortenproofright
\global\dimen2=\proofrulebreadth
\global\dimen3=\proofbelowshift
\global\dimen4=\proofdotseparation
\global\mscount=\proofdotnumber
% end the box
$\egroup  % NESTED ONE
%
% restore the values
\shortenproofleft=\dimen0
\shortenproofright=\dimen1
\proofrulebreadth=\dimen2
\proofbelowshift=\dimen3
\proofdotseparation=\dimen4
\proofdotnumber=\mscount
}

%=============================================================================
\def\proofover{% NESTED TWO
\eproofbit % NESTED ONE
\setbox\proofbelow=\hbox\bgroup % NESTED TWO
\let\wereinproofbit\proofover
$\displaystyle
}%
%
%=============================================================================
\def\proofoverdbl{% NESTED TWO
\eproofbit % NESTED ONE
\doubleprooftrue
\setbox\proofbelow=\hbox\bgroup % NESTED TWO
\let\wereinproofbit\proofoverdbl
$\displaystyle
}%
%
%=============================================================================
\def\proofoverdots{% NESTED TWO
\eproofbit % NESTED ONE
\proofdotstrue
\setbox\proofbelow=\hbox\bgroup % NESTED TWO
\let\wereinproofbit\proofoverdots
$\displaystyle
}%
%
%=============================================================================
\def\proofusing{% NESTED TWO
\eproofbit % NESTED ONE
\setbox\proofrulename=\hbox\bgroup % NESTED TWO
\let\wereinproofbit\proofusing
\kern0.3em$
}

%=============================================================================
\def\endprooftree{% NESTED TWO
\eproofbit % NESTED ONE
% \dimen0 =	length of proof rule
% \dimen1 =	indentation of conclusion wrt rule
% \dimen2 =	new \shortenproofleft, ie indentation of conclusion
% \dimen3 =	new \shortenproofright, ie
%		 space on right of conclusion to end of tree
% \dimen4 =	space on right of conclusion below rule
  \dimen5 =0pt% spread of hypotheses
% \dimen6, \dimen7 = height & depth of rule
%
% length of rule needed by proof above
\dimen0=\wd\proofabove \advance\dimen0-\shortenproofleft
\advance\dimen0-\shortenproofright
%
% amount of spare space below
\dimen1=.5\dimen0 \advance\dimen1-.5\wd\proofbelow
\dimen4=\dimen1
\advance\dimen1\proofbelowshift \advance\dimen4-\proofbelowshift
%
% conclusion sticks out to left of immediate hypotheses
\ifdim	\dimen1<0pt
\then	\advance\shortenproofleft\dimen1
	\advance\dimen0-\dimen1
	\dimen1=0pt
%	now it sticks out to left of tree!
	\ifdim  \shortenproofleft<0pt
        \then   \setbox\proofabove=\hbox{%
			\kern-\shortenproofleft\unhbox\proofabove}%
                \shortenproofleft=0pt
        \fi
\fi
%
% and to the right
\ifdim	\dimen4<0pt
\then	\advance\shortenproofright\dimen4
	\advance\dimen0-\dimen4
	\dimen4=0pt
\fi
%
% make sure enough space for label
\ifdim	\shortenproofright<\wd\proofrulename
\then	\shortenproofright=\wd\proofrulename
\fi
%
% calculate new indentations
\dimen2=\shortenproofleft \advance\dimen2 by\dimen1
\dimen3=\shortenproofright\advance\dimen3 by\dimen4
%
% make the rule or dots, with name attached
\ifproofdots
\then
	\dimen6=\shortenproofleft \advance\dimen6 .5\dimen0
	\setbox1=\vbox to\proofdotseparation{\vss\hbox{$\cdot$}\vss}
	\setbox0=\hbox{%
		\kern\dimen6
		$\vcenter to\proofdotnumber\proofdotseparation
			{\leaders\box1\vfill}$%
		\unhbox\proofrulename}%
\else	\dimen6=\fontdimen22\the\textfont2 % height of maths axis
	\dimen7=\dimen6
	\advance\dimen6by.5\proofrulebreadth
	\advance\dimen7by-.5\proofrulebreadth
	\setbox0=\hbox{%
		\kern\shortenproofleft
		\ifdoubleproof
		\then	\hbox to\dimen0{%
			$\mathsurround0pt\mathord=\mkern-6mu%
			\cleaders\hbox{$\mkern-2mu=\mkern-2mu$}\hfill
			\mkern-6mu\mathord=$}%
		\else	\vrule height\dimen6 depth-\dimen7 width\dimen0
		\fi
		\unhbox\proofrulename}%
	\ht0=\dimen6 \dp0=-\dimen7
\fi
%
% set up to centre outermost tree only
\let\doll\relax
\ifwasinsideprooftree
\then	\let\VBOX\vbox
\else	\ifmmode\else$\let\doll=$\fi
	\let\VBOX\vcenter
\fi
% this \vbox or \vcenter is the actual output:
\VBOX	{\baselineskip\proofrulebaseline \lineskip.2ex
	\expandafter\lineskiplimit\ifproofdots0ex\else-0.6ex\fi
	\hbox	spread\dimen5	{\hfi\unhbox\proofabove\hfi}%
	\hbox{\box0}%
	\hbox	{\kern\dimen2 \box\proofbelow}}\doll%
%
% pass new indentations out of scope
\global\dimen2=\dimen2
\global\dimen3=\dimen3
\egroup % NESTED ZERO
\ifonleftofproofrule
\then	\shortenproofleft=\dimen2
\fi
\shortenproofright=\dimen3
%
% some space on right and flag we've just made a tree
\onleftofproofrulefalse
\ifinsideprooftree
\then	\hskip.5em plus 1fil \penalty2
\fi
}

%==========================================================================
% IDEAS
% 1.	Specification of \shiftright and how to spread trees.
% 2.	Spacing command \m which causes 1em+1fil spacing, over-riding
%	exisiting space on sides of trees and not affecting the
%	detection of being on the left or right.
% 3.	Hack using \@currenvir to detect LaTeX environment; have to
%	use \aftergroup to pass \shortenproofleft/right out.
% 4.	(Pie in the sky) detect how much trees can be "tucked in"
% 5.	Discharged hypotheses (diagonal lines).


